Identifying outliers in astronomical images with unsupervised machine learning

Astronomical outliers, such as unusual, rare or unknown types of astronomical objects or phenomena, constantly lead to the discovery of genuinely unforeseen knowledge in astronomy. More unpredictable outliers will be uncovered in principle with the increment of the coverage and quality of upcoming survey data. However, it is a severe challenge to mine rare and unexpected targets from enormous data with human inspection due to a significant workload. Supervised learning is also unsuitable for this purpose since designing proper training sets for unanticipated signals is unworkable. Motivated by these challenges, we adopt unsupervised machine learning approaches to identify outliers in the data of galaxy images to explore the paths for detecting astronomical outliers. For comparison, we construct three methods, which are built upon the k-nearest neighbors (KNN), Convolutional Auto-Encoder (CAE)+ KNN, and CAE + KNN + Attention Mechanism (attCAE KNN) separately. Testing sets are created based on the Galaxy Zoo image data published online to evaluate the performance of the above methods. Results show that attCAE KNN achieves the best recall (78%), which is 53% higher than the classical KNN method and 22% higher than CAE+KNN. The efficiency of attCAE KNN (10 minutes) is also superior to KNN (4 hours) and equal to CAE+KNN(10 minutes) for accomplishing the same task. Thus, we believe it is feasible to detect astronomical outliers in the data of galaxy images in an unsupervised manner. Next, we will apply attCAE KNN to available survey datasets to assess its applicability and reliability.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

